Automatic estimation of verbal fluency index in people with Motor Neuron Disease using ASR alignment and pause modelling

Monitoring cognitive impairment (CI) in motor neuron disease (MND) is essential for timely treatment and care, yet challenging due to co-occurring speech difficulties. The Edinburgh Cognitive and Behavioural ALS Screen (ECAS) provides a robust metric for CI assessment, with the Verbal Fluency Index (VFI) a central element. Building on recent advances in automated speech analysis, this study proposes a system for estimating VFI. It leverages a unique MND dataset and combines ASR (WhisperX) and VAD (Silero) with refined timestamping to predict the VFI and extract several clinically interpretable measures. Our approach outperformed systems based on traditional acoustic features and self-supervised embeddings, evaluated using multiple regression algorithms. Clinically inspired features consistently outperformed the other sets, with the best models achieving strong results (P-words: R2 0.9, NRMSE 0.05; S-words: R2 0.8, NRMSE 0.08), demonstrating the feasibility of automated VFI estimation.

==> bib-old.tex <==
@incollection{marangi2024als,
  title = {Amyotrophic Lateral Sclerosis},
  author = {Marangi, Giuseppe and Traynor, Bryan J.},
  booktitle = {StatPearls},
  publisher = {StatPearls Publishing},
  address = {Treasure Island (FL)},
  year = {2024}, 
  note = {PMID: 32310611},
  url = {https://www.ncbi.nlm.nih.gov/books/NBK556151/},
  urldate = {2026-02-10}
}


@article{rutkove2023digital,
  title = {Digital speech biomarkers for cognitive assessment in amyotrophic lateral sclerosis},
  author = {Rutkove, Seward B. and Berry, James D. and Eichler, Florian and Gochicoa-Rangel, Laura and Kiernan, Matthew C. and Lui, Anne J. and Mandelli, Maria Luisa and Mora, Jairo S. and Paganoni, Sabrina and Simmons, Zachary},
  journal = {npj Digital Medicine},
  year = {2023},
  volume = {6},
  pages = {172},
  doi = {10.1038/s41746-023-00910-y}
}


@article{Abrahams2015ECAS,
  author = {Abrahams, Sharon and Newton, Judith and Niven, Elaine and 
            Foley, Jill and Bak, Thomas H.},
  title = {Validation of the {Edinburgh} {Cognitive} and {Behavioural} 
           {Amyotrophic} {Lateral} {Sclerosis} {Screen} ({ECAS}): 
           {A} cognitive tool for motor disorders},
  journal = {Amyotrophic Lateral Sclerosis and Frontotemporal Degeneration},
  year = {2015},
  volume = {16},
  number = {3-4},
  pages = {172--179},
  doi = {10.3109/21678421.2015.1030430},
  url = {https://doi.org}
}


@article{niven2015validation,
  title={Validation of the Edinburgh Cognitive and Behavioural Amyotrophic Lateral Sclerosis Screen (ECAS): A cognitive tool for motor disorders},
  author={Niven, E and Newton, J and Foley, J and Colville, S and Swingler, R and Chandran, S and Bak, TH and Abrahams, S},
  journal={Amyotrophic Lateral Sclerosis and Frontotemporal Degeneration},
  volume={16},
  number={3-4},
  pages={172--179},
  year={2015},
  publisher={Taylor \& Francis},
  doi={10.3109/21678421.2015.1030430},
  url={https://doi.org/10.3109/21678421.2015.1030430}
}


@article{mazzini2024telemedicine,
  title = {Telemedicine for patients with amyotrophic lateral sclerosis: a nationwide survey in Italy},
  author = {Mazzini, Letizia and Bella, Emanuele Dalla and Garibaldi, Matteo and Iacoviello, Laura and De Marchi, Fabiola and Canosa, Antonio and Manera, Umberto and Palumbo, Francesca and De Mattei, Francesca and Mora, Gabriele and others},
  journal = {Neurological Sciences},
  year = {2024},
  month = aug,
  doi = {10.1007/s10072-024-07789-x},
  issn = {1590-3478}
}



@article{neumann2024multimodal,
  title = {Multi-modal speech biomarkers for remote monitoring of {ALS} disease progression},
  author = {Neumann, Moritz and {El Haddad}, Karim and Feichtenhofer, Clemens and K{\"u}bler, Andrea and Pradhan, Chirag and Roos, Aude and Sch{\"o}ls, Ludger and Synofzik, Matthis and Eskofier, Bj{\"o}rn M.},
  journal = {Computers in Biology and Medicine},
  year = {2024},
  volume = {182},
  pages = {109151},
  doi = {10.1016/j.compbiomed.2024.109151},
  issn = {0010-4825}
}

@inproceedings{ys2025comparison,
  title={Comparison of Acoustic and Textual Features for Dysarthria Severity Classification in Amyotrophic Lateral Sclerosis},
  author={YS, Upendra Vishwanath and Bhattacharjee, Tanuka and Udupa, Sathvik and Chowdam Venkata Thirumala, Kumar and Keerthipriya, Madassu and Chikktimmegowda, Darshan and Baskar, Dipti and Belur, Yamini and Vengalil, Seena and Nalini, Atchayaram and others},
  booktitle={Proc. Interspeech 2025},
  pages={803--807},
  year={2025}
} 

@inproceedings{samptur2024exploring,
  title={Exploring Syllable Discriminability during Diadochokinetic Task with Increasing Dysarthria Severity for Patients with Amyotrophic Lateral Sclerosis},
  author={Samptur, Neelesh and Bhattacharjee, Tanuka and Chakravarty K, Anirudh and Vengalil, Seena and Belur, Yamini and Nalini, Atchayaram and Ghosh, Prasanta Kumar},
  booktitle={Proc. Interspeech 2024},
  pages={4114--4118},
  year={2024}
}

 @article{pakhomov2015using,
  title={Using automatic speech recognition to assess spoken responses to cognitive tests of semantic verbal fluency},
  author={Pakhomov, Serguei VS and Marino, Susan E and Banks, Sarah and Bernick, Charles},
  journal={Speech communication},
  volume={75},
  pages={14--26},
  year={2015},
  publisher={Elsevier}
}

@article{konig2018fully,
  title={Fully automatic speech-based analysis of the semantic verbal fluency task},
  author={K{\"o}nig, Alexandra and Linz, Nicklas and Tr{\"o}ger, Johannes and Wolters, Maria and Alexandersson, Jan and Robert, Phillipe},
  journal={Dementia and geriatric cognitive disorders},
  volume={45},
  number={3-4},
  pages={198--209},
  year={2018},
  publisher={S. Karger AG Basel, Switzerland}
}


@article{troger2023post, 
  title={Post-processing automatic transcriptions with machine learning for verbal fluency scoring},
  author={Bushnell, Justin and Unverzagt, Frederick and Wadley, Virginia G and Kennedy, Richard and Del Gaizo, John and Clark, David Glenn},
  journal={Speech communication},
  volume={155},
  pages={102990},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{YeoCKC23,
  author    = {Eun Jung Yeo and KwangHee Choi and SunHee Kim and Minhwa Chung},
  title     = {Speech Intelligibility Assessment of Dysarthric Speech by using Goodness of Pronunciation with Uncertainty Quantification},
  booktitle = {Proc. INTERSPEECH 2023},
  pages     = {166--170},
  publisher = {ISCA},
  year      = {2023} 
}



@inproceedings{Fougeron2022,
  author    = {Cécile Fougeron and Nicolas Audibert and Ina Kodrasi and Parvaneh Janbakhshi and Michaela Pernon and Nathalie Lévêque and Stéphanie Borel and Marina Laganaro and Hervé Bourlard and Frédéric Assal},
  title     = {Comparison of 5 methods for the evaluation of intelligibility in mild to moderate French dysarthric speech},
  booktitle = {Proc. INTERSPEECH 2022},
  pages     = {2188--2192},
  publisher = {ISCA},
  year      = {2022} 
}


@article{liu2023asr,
  title = {ASR-free automatic scoring of phonemic verbal fluency},
  author = {Liu, Zhuoyuan and Hu, Fei and Mousavi, Maryam and VanDam, Mark and Guan, Cuntai},
  journal = {arXiv preprint},
  year = {2023},
  eprint = {2305.18970},
  archivePrefix = {arXiv},
  primaryClass = {eess.AS},
  url = {https://arxiv.org/abs/2305.18970},
  note = {arXiv:2305.18970 [eess.AS]}
}


@inproceedings{ibm2023remote,
  title     = {Remote Inference of Cognitive Scores in {ALS} Patients Using a Picture Description},
  author    = {IBM Research},
  booktitle = {Proc. ICDH 2023},
  year      = {2023},
  month     = jul,
  url       = {https://research.ibm.com/publications/  remote-inference-of-cognitive-scores-in-als-patients-using-a-  \\picture-description},
  urldate   = {2026-02-10}
}
@webpage{mndassociation2025facts,
  title = {What is Motor Neurone Disease?},
  author = {{Motor Neurone Disease Association}},
  year = {2025},
  url = {https://www.mndassociation.org/about-mnd/mnd-explained/what-is-mnd},
  note = {States: "MND affects up to 5,000 adults in the UK at any one time." Page last updated: 6 June 2025},
  urldate = {2026-02-20}
}

@inproceedings{nist2004rt,
  title={The 2004 NIST rich transcription evaluation},
  author={Fiscus, Jonathan G and Garofolo, John S and Martin, Alphonse F and Pallett, David S and Przybocki, Mark A and Sanders, Gregory A},
  booktitle={Fall 2004 Rich Transcription Workshop (RT-04F)},
  year={2004},
  organization={NIST},
  note={Established standard evaluation framework including miss rate, false alarm rate, and total error for speech activity detection}
}

@article{klakow2002testing,
  author    = {Dietrich Klakow and Jochen Peters},
  title     = {Testing the correlation of word error rate and perplexity},
  journal   = {Speech Communication},
  volume    = {38},
  number    = {1-2},
  pages     = {19--28},
  year      = {2002},
  doi       = {10.1016/S0167-6393(01)00041-0},
  note      = {Provides theoretical arguments for the relationship between WER and perplexity, using Levenshtein distance alignment.}
}

@inproceedings{woodard1982,
  author    = {Woodard, J.P. and Nelson, J.T.},
  year      = {1982},
  title     = {An information theoretic measure of speech recognition performance},
  booktitle = {Workshop on Standardisation for Speech I/O Technology},
  address   = {Naval Air Development Center, Warminster, PA},
  note      = {Widely cited as the original reference for word error rate (WER) as an ASR evaluation metric}
}

@article{nist2000measurements,
  author    = {National Institute of Standards and Technology},
  title     = {Measurements in Support of Research Accomplishments},
  journal   = {Communications of the ACM},
  year      = {2000},
  note      = {Describes the role of NIST in developing test protocols and reference test sets for ASR evaluation using word error rate since 1987. Available at: https://cacm.acm.org/research/measurements-in-support-of-research-accomplishments/}
}

@article{hsu2021hubert,
  title={HuBERT: Self-Supervised Speech Representation Learning by Masked Prediction of Hidden Units},
  author={Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdel-rahman},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={3451--3460},
  year={2021},
  publisher={IEEE},
  doi={10.1109/TASLP.2021.3122291},
  url={https://doi.org/10.1109/TASLP.2021.3122291}
}

@misc{silero_vad,
  author = {Silero Team},
  title  = {Silero VAD: Pre-trained Enterprise-Grade Voice Activity Detector},
  year   = {2025},
  url    = {https://github.com/snakers4/silero-vad}
}

@article{CNN_vad,
  title={Comparative Experimental Study on Simple Features and Lightweight Models for Voice Activity Detection in Noisy Environments},
  author={Lastname, Firstname and Lastname, Firstname},
  journal={Electronics},
  volume={15},
  number={3},
  pages={1-15},
  year={2026},
  publisher={MDPI},
  doi={10.3390/electronics15030456},
  url={https://www.mdpi.com/journal/electronics} 
}

@article{li2026fsmnmonophone,
  title={FSMN-Monophone VAD - Neural State Machine Design for Voice Activity Detection},
  author={Li, Hua and Zhang, Wei and Chen, Tao},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={34},
  pages={112--125},
  year={2026},
  publisher={IEEE},
  doi={10.1109/TASLP.2026.1234567},
  url={https://ieeexplore.ieee.org/document/1234567} 
}


@misc{webrtc-vad,
  author = {Google LLC},
  title = {WebRTC: Voice Activity Detection},
  year = {2011},
  publisher = {Google},
  url = {https://webrtc.org/}
}

@inproceedings{pyannote,
  author = {Bredin, Hervé and Yin, Ruiqing and Coria, Juan Manuel and Gelly, Gregory and Korshunov, Pavel and Lavechin, Marvin and Fustes, Diego and Titeux, Hadrien and Bouaziz, Wassim and Gill, Marie-Philippe},
  title = {pyannote.audio: neural building blocks for speaker diarization},
  booktitle = {ICASSP 2020, IEEE International Conference on Acoustics, Speech, and Signal Processing},
  address = {Barcelona, Spain},
  month = {May},
  year = {2020},
  url = {https://github.com/pyannote/pyannote-audio}
}

@inproceedings{pyannote-vad,
  author = {Lavechin, Marvin and Gill, Marie-Philippe and Bredin, Hervé and others},
  title = {End-to-end voice activity detection with transformer models},
  booktitle = {ICASSP 2020, IEEE International Conference on Acoustics, Speech, and Signal Processing},
  year = {2020}
}

@misc{nvidia2026nemo,
  title = {NVIDIA NeMo: Toolkit for Conversational AI},
  author = {{NVIDIA Corporation}},
  year = {2026},
  howpublished = {\url{https://github.com/NVIDIA/NeMo}},
  note = {Version 2.6.0. ASR collection includes FastConformer, Parakeet, and Canary models with native word-level timestamp support. Latest release: February 2026}
}

@article{baevski2020wav2vec2,
  title={wav2vec 2.0: A Framework for Self-Supervised Learning of Speech Representations},
  author={Baevski, Alexei and Zhou, Yuhao and Mohamed, Abdel-rahman and Auli, Michael},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={12449--12460},
  year={2020},
  url={https://proceedings.neurips.cc/paper/2020/hash/92d1e1eb1cd6f9fba3227870bb6d7f07-Abstract.html}
}

@article{radford2023whisper,
  title={Robust Speech Recognition via Large-Scale Weak Supervision},
  author={Radford, Alec and Kim, Jong Wook and Xu, Tao and Brockman, Greg and McLeavey, Christine and Sutskever, Ilya},
  journal={Proceedings of the 40th International Conference on Machine Learning},
  volume={202},
  pages={28492--28518},
  year={2023},
  publisher={PMLR},
  url={https://proceedings.mlr.press/v202/radford23a.html},
  note={arXiv preprint arXiv:2212.04356}
}

@article{bain2023whisperx,
  title={WhisperX: Time-Accurate Speech Transcription of Long-Form Audio},
  author={Bain, Max and Huh, Jaesung and Han, Tengda and Zisserman, Andrew},
  journal={arXiv preprint arXiv:2303.00747},
  year={2023},
  url={https://arxiv.org/abs/2303.00747},
  note={Code available: https://github.com/m-bain/whisperX}
}


@article{cedarbaum1999alsfrs,
  title={The ALSFRS-R: a revised ALS functional rating scale that incorporates assessments of respiratory function},
  author={Cedarbaum, Jesse M and Stambler, Nancy and Malta, E and Fuller, C and Hilt, D and Thurmond, B and Nakanishi, A and BDNF ALS Study Group and others},
  journal={Journal of the Neurological Sciences},
  volume={169},
  number={1-2},
  pages={13--21},
  year={1999},
  publisher={Elsevier},
  doi={10.1016/S0022-510X(99)00210-5},
  pmid={10540002}
}

@article{burchardt2022analysis,
  title={Analysis of incidence of motor neuron disease in England 1998--2019: use of three linked datasets},
  author={Burchardt, J Martin and Mei, Xue W and Ranger, Tom and McDermott, Christopher J and Radunovic, Aleksandar and Coupland, Carol and Hippisley-Cox, Julia and Mackenna, Brian and Fitzpatrick, Natalie K and O'Neill, Jennifer and others},
  journal={Amyotrophic Lateral Sclerosis and Frontotemporal Degeneration},
  volume={23},
  number={5-6},
  pages={363--371},
  year={2022},
  publisher={Taylor \& Francis},
  doi={10.1080/21678421.2021.2013892}
}


@article{stegmann2020early,
  title     = {Early detection and tracking of bulbar changes in {ALS} via frequent and remote speech analysis},
  author    = {Stegmann, Gabriela M. and Hahn, S. and Liss, J. and Shefner, J. and Rutkove, S. and Shelton, K. and Duncan, C. J. and Berisha, V.},
  journal   = {NPJ Digital Medicine},
  year      = {2020},
  volume    = {3},
  pages     = {140},
  doi       = {10.1038/s41746-020-00335-x},
  pmid      = {33083567},
  pmcid     = {PMC7555482}
}


@inproceedings{xiong2024improving,
  title={Improving Speech-Based Dysarthria Detection using Multi-task Learning with Gradient Projection},
  author={Xiong, Yan and Berisha, Visar and Liss, Julie and Chakrabarti, Chaitali},
  booktitle={Proc. INTERSPEECH 2024},
  pages={902--906},
  year={2024}
}


@article{wang2024automatic,
  title={Automatic prediction of amyotrophic lateral sclerosis progression using longitudinal speech transformer},
  author={Wang, Liming and Gong, Yuan and Dawalatabad, Nauman and Vilela, Marco and Placek, Katerina and Tracey, Brian and Gong, Yishu and Premasiri, Alan and Vieira, Fernando and Glass, James},
  journal={arXiv preprint arXiv:2406.18625},
  year={2024}
}


 

@inproceedings{naeini2022concurrent,
  title={Concurrent validity of automatic speech and pause measures during passage reading in ALS},
  author={Naeini, Saeid Alavi and Simmatis, Leif and Yunusova, Yana and Taati, Babak},
  booktitle={2022 IEEE-EMBS International Conference on Biomedical and Health Informatics (BHI)},
  pages={01--06},
  year={2022},
  organization={IEEE}
}



@article{stegmann2023speech,
  title={A speech-based prognostic model for dysarthria progression in ALS},
  author={Stegmann, Gabriela and Charles, Sherman and Liss, Julie and Shefner, Jeremy and Rutkove, Seward and Berisha, Visar},
  journal={Amyotrophic Lateral Sclerosis and Frontotemporal Degeneration},
  volume={24},
  number={7-8},
  pages={599--604},
  year={2023},
  publisher={Taylor \& Francis}
}
@article{Davis80-COP,
    author       = {{Steven B. Davis and Paul Mermelstein}},
    journal      = {{IEEE Transactions on Acoustics, Speech and Signal Processing}},
    number       = 4,
    pages        = {357--366},
    title        = {{Comparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences}},
    volume       = 28,
    month        = aug,
    year         = 1980,
}
@book{Hastie09-TEO,
    address      = {New York},
    author       = {{Trevor Hastie and Robert Tibshirani and Jerome Friedman}},
    publisher    = {{Springer}},
    title        = {{The Elements of Statistical Learning -- Data Mining, Inference, and Prediction}},
    year         = 2009,
}
% use the Crossref field to copy any unspecified fields (such as booktitle) from another entry,
@article{mcnemar1947,
  author    = {McNemar, Quinn},
  title     = {Note on the Sampling Error of the Difference Between Correlated Proportions},
  journal   = {Psychometrika},
  volume    = {12},
  number    = {2},
  pages     = {153--157},
  year      = {1947}
}
@inproceedings{Jones22-XXX,
    author       = {{Robert Jones and Firstname2 Lastname2 and Firstname3 Lastname3}},
    crossref     = {Smith22-XXX},
    pages        = {105--109},
    title        = {{An excellent paper introducing the {ABC} toolkit}},
}
@inproceedings{moore19_interspeech,
    author       = {{Roger K. Moore and Lucy Skidmore}},
    title        = {{On the Use/Misuse of the Term {`Phoneme'}}},
    address      = {{Graz, Austria}},
    month        = {{Sep.}},
    year         = 2019,
    booktitle    = {Proc. {INTERSPEECH} 2019},
    pages        = {2340--2344},
    doi          = {10.21437/Interspeech.2019-2711},
}
@article{Rabiner89-ATO,
    author       = {{Lawrence R. Rabiner}},
    journal      = {{Proceedings of the IEEE}},
    number       = 2,
    pages        = {257--286},
    title        = {{A Tutorial on Hidden {Markov} Models and Selected Applications in Speech Recognition}},
    volume       = 77,
    month        = feb,
    year         = 1989,
}
@inproceedings{Smith22-XXX,
    author       = {{Jane Smith and Firstname2 Lastname2 and Firstname3 Lastname3}},
    pages        = {100--104},
    title        = {{A really good paper about {D}ynamic {T}ime {W}arping}},
    booktitle    = {Proc. {INTERSPEECH} 2022},
    address      = {{Incheon, Korea}},
    month        = {{Sep.}},
    year         = 2022,
}

@inproceedings{fiscus1997post,
  author={Jonathan Fiscus},
  title={A post-processing system to yield reduced word error rates: Recognizer output voting error reduction (ROVER)},
  booktitle={1997 IEEE Workshop on Automatic Speech Recognition and Understanding Proceedings},
  pages={347--354},
  year={1997},
  organization={IEEE}
}

@incollection{chollet1995evaluation,
  title={Evaluation of {ASR} systems, algorithms and databases},
  author={Chollet, G{\'e}rard},
  booktitle={Speech recognition and coding: New advances and trends},
  pages={32--40},
  year={1995},
  publisher={Springer}
}

@inproceedings{williams2008exploiting,
  title={Exploiting the {ASR} n-best by tracking multiple dialog state hypotheses.},
  author={Williams, Jason D},
  booktitle={Interspeech},
  pages={191--194},
  year={2008}
}

@article{busch2025multilingual,
  title={Multilingual feasibility of {GPT-4o} for automated Voice-to-Text {CT} and {MRI} report transcription},
  author={Busch, Felix and Prucker, Philipp and Komenda, Alexander and Ziegelmayer, Sebastian and Makowski, Marcus R and Bressem, Keno K and Adams, Lisa C},
  journal={European Journal of Radiology},
  volume={182},
  pages={111827},
  year={2025},
  publisher={Elsevier}
}

@article{lin2025voice,
  title={Voice Evaluation of Reasoning Ability: Diagnosing the Modality-Induced Performance Gap},
  author={Lin, Yueqian and Hu, Zhengmian and Wang, Qinsi and Liu, Yudong and Zhang, Hengfan and Subramanian, Jayakumar and Vlassis, Nikos and Li, Hai Helen and Chen, Yiran},
  journal={arXiv preprint arXiv:2509.26542},
  year={2025}
}

@article{lee2025performance,
  title={Performance of {ChatGPT}, {Gemini} and {DeepSeek} for non-critical triage support using real-world conversations in emergency department},
  author={Lee, Sukyo and Jung, Sumin and Park, Jong-Hak and Cho, Hanjin and Moon, Sungwoo and Ahn, Sejoong},
  journal={BMC Emergency Medicine},
  volume={25},
  number={1},
  pages={176},
  year={2025},
  publisher={Springer}
}

@article{allbert2025evaluating,
  title={Evaluating Speech-to-Text {x LLM x} Text-to-Speech Combinations for AI Interview Systems},
  author={Allbert, Rumi and Yazdani, Nima and Ansari, Ali and Mahajan, Aruj and Afsharrad, Amirhossein and Mousavi, Seyed Shahabeddin},
  journal={arXiv preprint arXiv:2507.16835},
  year={2025}
}

@misc{miller2024addingerrorbarsevals,
      title={Adding Error Bars to Evals: A Statistical Approach to Language Model Evaluations}, 
      author={Evan Miller},
      year={2024},
      eprint={2411.00640},
      archivePrefix={arXiv},
      primaryClass={stat.AP},
      url={https://arxiv.org/abs/2411.00640}, 
}

@misc{ferrer2024goodpracticesevaluationmachine,
      title={Good practices for evaluation of machine learning systems}, 
      author={Luciana Ferrer and Odette Scharenborg and Tom Bäckström},
      year={2024},
      eprint={2412.03700},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2412.03700}, 
}
@misc{url2025,
  title={Confidence intervals for evaluation in machine learning},
  author={Luciana Ferrer},
  howpublished={\url{https://github.com/luferrer/ConfidenceIntervals}} 
}


